Causal Concept Graph Models: Beyond Causal Opacity in Deep Learning

Causal opacity denotes the difficulty in understanding the "hidden" causal structure underlying the decisions of deep neural network (DNN) models. This leads to the inability to rely on and verify state-of-the-art DNN-based systems, especially in high-stakes scenarios. For this reason, circumventing causal opacity in DNNs represents a key open challenge at the intersection of deep learning, interpretability, and causality. This work addresses this gap by introducing Causal Concept Graph Models (Causal CGMs), a class of interpretable models whose decision-making process is causally transparent by design. Our experiments show that Causal CGMs can: (i) match the generalisation performance of causally opaque models, (ii) enable human-in-the-loop corrections to mispredicted intermediate reasoning steps, boosting not just downstream accuracy after corrections but also the reliability of the explanations provided for specific instances, and (iii) support the analysis of interventional and counterfactual scenarios, thereby improving the model's causal interpretability and supporting the effective verification of its reliability and fairness.

==> figs/tikz_pics.tex <==
% Define global variables for separations
\newlength{\nodesep}
\setlength{\nodesep}{1cm} % distance between nodes
\newlength{\innersep}
\setlength{\innersep}{2pt}  % inner separation within nodes
\newlength{\sep}
\setlength{\sep}{1.3cm}    % uniform separation for both vertical and horizontal
\newcommand{\vsep}{.9cm}
\newcommand{\hsep}{.9cm}
    
% \newcommand{\scm}{
% \begin{tikzpicture}
%     % Define observable nodes with circles
%     \node[circle, draw, inner sep=\innersep] (c) at (0,0) {$c_1$};
%     \node[circle, draw, inner sep=\innersep] (y) at (\sep,0) {$c_2$};

%     \node at (\sep,0.5) {$f(c_1, u_2)$};

%     % Define other nodes with squares
%     \node[rectangle, draw, inner sep=\innersep] (uc) at (0,-\nodesep) {$u_1$};
%     \node[rectangle, draw, inner sep=\innersep] (uy) at (\sep,-\nodesep) {$u_2$};
    
%     % Draw arrows
%     \draw[->, dashed] (uc) -- (c);
%     \draw[->, dashed] (uy) -- (y);
%     \draw[->] (c) -- (y);
% \end{tikzpicture}
% }

% \newcommand{\scmdo}{
% \begin{tikzpicture}
%     % Define observable nodes with circles
%     \node[circle, draw, inner sep=\innersep] (c) at (0,0) {$c_1$};
%     \node[circle, draw, inner sep=\innersep] (y) at (\sep,0) {$c_2$};

%     \node at (\sep,0.5) {do$(c_2 = \kappa)$};

%     % Define other nodes with squares
%     \node[rectangle, draw, inner sep=\innersep] (uc) at (0,-\nodesep) {$u_1$};
%     \node[rectangle, draw, inner sep=\innersep] (uy) at (\sep,-\nodesep) {$u_2$};
    
%     % Draw arrows
%     \draw[->, dashed] (uc) -- (c);
%     % \draw[->, dashed] (uy) -- (y);
%     % \draw[->] (c) -- (y);
% \end{tikzpicture}
% }

\newcommand{\scmcheckmark}{
\begin{tikzpicture}
    % Define epsilon nodes at the top
    \node[rectangle, draw, inner sep=\innersep] (e0) at (0,0) {$\epsilon_0$};
    \node[rectangle, draw, inner sep=\innersep] (e3) at (\hsep,0) {$\epsilon_3$};

    % Define c0 and c3 below epsilon nodes
    \node[circle, draw, inner sep=\innersep] (c0) at (0,-\vsep) {$c_0$};
    \node[circle, draw, inner sep=\innersep] (c3) at (\hsep,-\vsep) {$c_3$};

    % Define c1 below c0 and c3
    \node[circle, draw, inner sep=\innersep] (c1) at (\hsep,-2*\vsep) {$c_1$};

    % Define c2 at the bottom
    \node[circle, draw, inner sep=\innersep] (c2) at (\hsep/2,-3*\vsep) {$c_2$};
    
    % Draw arrows
    \draw[->] (e0) -- (c0);
    \draw[->] (e3) -- (c3);
    \draw[->] (c0) -- (c2);
    \draw[->] (c3) -- (c1);
    \draw[->] (c1) -- (c2);
\end{tikzpicture}
}




\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\tikzset{
    % main node/.style = {circle, draw=none, thick, fill=gray!20},
    % message node/.style = {rectangle, draw=none, thick, fill=green!20, align=center},
    % concept message node/.style = {rectangle, draw=none, thick, fill=blue!20, align=center},
    % agg node/.style = {circle, draw=none, thick, fill=blue!20},
    % arrow style/.style = {dotted, thick,-{Stealth[]},shorten >=1pt},
    % big arrow/.style={line width=1mm, shorten >=1pt, color=gray},
    square1/.style={draw, fill=gray!20, minimum size=.3cm},
    square2/.style={draw, fill=gray!50, minimum size=.3cm},
    square3/.style={draw, fill=gray!100, minimum size=.3cm},
    true/.style = {circle, draw=none, thick, fill=green!50, minimum width=.5cm, minimum height=.5cm, inner sep=0pt},
    false/.style = {circle, draw=none, thick, fill=red!50, minimum width=.5cm, minimum height=.5cm, inner sep=0pt},
    plain/.style = {circle, draw, thick, fill=none, minimum width=.5cm, minimum height=.5cm, inner sep=0pt},
    arrowstyle/.style={->, thick, rounded corners},
    arrowstyledash/.style={->, thick, rounded corners, dash pattern=on 2pt off .6pt, gray},
    adjweight/.style={->, dashed, line width=.1mm, color=blue!50},
    adjweightbig/.style={->, line width=.6mm, color=blue!50},
    cembtrue1/.style={draw, fill=green!20, minimum size=.3cm},
    cembtrue2/.style={draw, fill=green!50, minimum size=.3cm},
    cembtrue3/.style={draw, fill=green!100, minimum size=.3cm},
    cembfalse1/.style={draw, fill=red!20, minimum size=.3cm},
    cembfalse2/.style={draw, fill=red!50, minimum size=.3cm},
    cembfalse3/.style={draw, fill=red!100, minimum size=.3cm},
    operation/.style={draw, thick, fill=blue!20, minimum size=0.6cm,  rounded corners=5pt, inner sep=1pt, outer sep=0pt, align=center},
}
\newcommand{\CCEMtrain}{
\begin{tikzpicture}[
    node distance = 1.3cm,
]

% Input Nodes
\node[inner sep=0pt] (img_dsprites) {\includegraphics[width=2cm]{figs/h_dsprites.png}};
\node[above=1.8cm of img_dsprites.north, align=center] (label) {
    \textbf{Input}
};

% input encoder
\node[operation, minimum width=2cm, minimum height=4cm] (zeta) [right=1cm of img_dsprites] {\textbf{Exogenous}\\\textbf{Encoder}\\$\zeta$};

% Arrows from input to encoder
\draw[arrowstyle] (img_dsprites) to [] (zeta);

% Context
\node[square1] (sq11) [right=1cm of zeta, yshift=2cm] {};
\node[square2] (sq12) [right=0cm of sq11] {};
\node[square3] (sq13) [right=0cm of sq12] {};
\node[above=0cm of sq12.north] (label) {RedHeart};
\node[square1] (sq21) [below=1cm of sq11] {};
\node[square2] (sq22) [right=0cm of sq21] {};
\node[square3] (sq23) [right=0cm of sq22] {};
\node[above=0cm of sq22.north] (label) {White};
\node[square1] (sq31) [below=1cm of sq21] {};
\node[square2] (sq32) [right=0cm of sq31] {};
\node[square3] (sq33) [right=0cm of sq32] {};
\node[above=0cm of sq32.north] (label) {Square};
\node[square1] (sq41) [below=1cm of sq31] {};
\node[square2] (sq42) [right=0cm of sq41] {};
\node[square3] (sq43) [right=0cm of sq42] {};
\node[above=0cm of sq42.north] (label) {Top};
\node[above=.5cm of sq12.north, align=center] (label) {
    \textbf{Exogenous}\\
    \textbf{Variables}
};
\node[below=0.5cm of sq42.south, align=center] (label) {$\hat{\mathbf{u}}_i$};

% Arrows from encoder to exogenous
\draw[arrowstyle] (zeta) to [] (sq11);
\draw[arrowstyle] (zeta) to [] (sq21);
\draw[arrowstyle] (zeta) to [] (sq31);
\draw[arrowstyle] (zeta) to [] (sq41);

% scoring function
\node[operation] (s1) [right= of sq13] {$s$};
\node[operation] (s2) [right= of sq23] {$s$};
\node[operation] (s3) [right= of sq33] {$s$};
\node[operation] (s4) [right= of sq43] {$s$};

% Arrows from contexts to scoring
\draw[arrowstyle] (sq13) to [] (s1);
\draw[arrowstyle] (sq23) to [] (s2);
\draw[arrowstyle] (sq33) to [] (s3);
\draw[arrowstyle] (sq43) to [] (s4);

% concept predictions
\node[true] (c1) [right= of s1] {\cmark};
\node[false] (c2) [right= of s2] {\xmark};
\node[false] (c3) [right= of s3] {\xmark};
\node[true] (c4) [right= of s4] {\cmark};
\node[above=.3cm of c1.north, align=center] (label) {
    \textbf{Endogenous}\\
    \textbf{Copies}
};
\node[below=0.4cm of c4.south, align=center] (label) {$\hat{v}_i'$};

% Arrows from scoring to predictions
\draw[arrowstyle] (s1) to [] (c1);
\draw[arrowstyle] (s2) to [] (c2);
\draw[arrowstyle] (s3) to [] (c3);
\draw[arrowstyle] (s4) to [] (c4);

% concept embedding function
\node[operation] (ceop1) [right= of c1] {$\omega$};
\node[operation] (ceop2) [right= of c2] {$\omega$};
\node[operation] (ceop3) [right= of c3] {$\omega$};
\node[operation] (ceop4) [right= of c4] {$\omega$};

% Arrows from concept predictions to concept embedding function
\draw[arrowstyle] (c1) to [] (ceop1);
\draw[arrowstyle] (c2) to [] (ceop2);
\draw[arrowstyle] (c3) to [] (ceop3);
\draw[arrowstyle] (c4) to [] (ceop4);

% concept embeddings
\node[cembtrue1] (ce11) [right= of ceop1] {};
\node[cembtrue2] (ce12) [right=0cm of ce11] {};
\node[cembtrue3] (ce13) [right=0cm of ce12] {};
\node[above=0cm of ce12.north] (label) {RedHeart};
\node[cembfalse1] (ce21) [below=1cm of ce11] {};
\node[cembfalse2] (ce22) [right=0cm of ce21] {};
\node[cembfalse3] (ce23) [right=0cm of ce22] {};
\node[above=0cm of ce22.north] (label) {White};
\node[cembfalse1] (ce31) [below=1cm of ce21] {};
\node[cembfalse2] (ce32) [right=0cm of ce31] {};
\node[cembfalse3] (ce33) [right=0cm of ce32] {};
\node[above=0cm of ce32.north] (label) {Square};
\node[cembtrue1] (ce41) [below=1cm of ce31] {};
\node[cembtrue2] (ce42) [right=0cm of ce41] {};
\node[cembtrue3] (ce43) [right=0cm of ce42] {};
\node[above=0cm of ce42.north] (label) {Top};
\node[above=.4cm of ce12.north, align=center] (label) {
    \textbf{Endogenous}\\
    \textbf{Embeddings}
};
\node[below=0.5cm of ce42.south, align=center] (label) {$\hat{\mathbf{v}}_i$};

% Arrows from concept predictions to embeddings
\draw[arrowstyle] (ceop1) to [] (ce11);
\draw[arrowstyle] (ceop2) to [] (ce21);
\draw[arrowstyle] (ceop3) to [] (ce31);
\draw[arrowstyle] (ceop4) to [] (ce41);
\draw[arrowstyle] (sq12.south) -- ++(0,-0.4) -| (ceop1.south);
\draw[arrowstyle] (sq22.south) -- ++(0,-0.4) -| (ceop2.south);
\draw[arrowstyle] (sq32.south) -- ++(0,-0.4) -| (ceop3.south);
\draw[arrowstyle] (sq42.south) -- ++(0,-0.4) -| (ceop4.south);

% % aggregation functions
% \node[operation] (agg1) [right=1cm of ce13] {$\oplus$};
% \node[operation] (agg2) [right=1cm of ce23] {$\oplus$};
% \node[operation] (agg3) [right=1cm of ce33] {$\oplus$};
% \node[operation] (agg4) [right=1cm of ce43] {$\oplus$};

% % concept embeddings posteriors
% \node[square1] (cep11) [right= of agg1] {};
% \node[square3] (cep12) [right=0cm of cep11] {};
% \node[above=0cm of cep11.north] (label) {RedHeart};
% \node[square1] (cep21) [below=1cm of cep11] {};
% \node[square3] (cep22) [right=0cm of cep21] {};
% \node[above=0cm of cep21.north] (label) {White};
% \node[square1] (cep31) [below=1cm of cep21] {};
% \node[square3] (cep32) [right=0cm of cep31] {};
% \node[above=0cm of cep31.north] (label) {Square};
% \node[square1] (cep41) [below=1cm of cep31] {};
% \node[square3] (cep42) [right=0cm of cep41] {};
% \node[above=0cm of cep41.north] (label) {Top};
% \node[below=0.5cm of cep42.south, align=center] (label) {$\hat{\mathbf{c}}_i$};
% \node[below=0.5cm of cep42.south, align=center, xshift=-1.8cm] (label) {$A$};
% \node[above=.8cm of cep11.north, align=center] (label) {
%     \textbf{Concept}\\
%     \textbf{Messages}
% };

% scoring function
\node[operation] (f1) [right=1cm of ce13] {$f_r$};
\node[operation] (f2) [right=1cm of ce23] {$f_w$};
\node[operation] (f3) [right=1cm of ce33] {$f_s$};
\node[operation] (f4) [right=1cm of ce43] {$f_t$};

% Arrows from concept embeddings to their posteriors
\draw[adjweight] (ce13) to [] (f2);
\draw[adjweight] (ce13) to [] (f3);
\draw[adjweight] (ce13) to [] (f4);
\draw[adjweightbig] (ce23) to [] (f1);
\draw[adjweight] (ce23) to [] (f3);
\draw[adjweight] (ce23) to [] (f4);
\draw[adjweightbig] (ce33) to [] (f1);
\draw[adjweight] (ce33) to [] (f2);
\draw[adjweight] (ce33) to [] (f4);
\draw[adjweight] (ce43) to [] (f1);
\draw[adjweightbig] (ce43) to [] (f2);
\draw[adjweight] (ce43) to [] (f3);

% % Arrows from aggregation functions to concept posteriors
% \draw[arrowstyle] (agg1) to [] (cep11);
% \draw[arrowstyle] (agg2) to [] (cep21);
% \draw[arrowstyle] (agg3) to [] (cep31);
% \draw[arrowstyle] (agg4) to [] (cep41);


% % Arrows from concept posteriors to predictions
% \draw[arrowstyle] (cep12) to [] (f1);
% \draw[arrowstyle] (cep22) to [] (f2);
% \draw[arrowstyle] (cep32) to [] (f3);
% \draw[arrowstyle] (cep42) to [] (f4);

% task predictions
\node[true] (y1) [right= of f1] {\cmark};
\node[false] (y2) [right= of f2] {\xmark};
\node[false] (y3) [right= of f3] {\xmark};
\node[true] (y4) [right= of f4] {\cmark};
\node[above=.35cm of y1.north, align=center] (label) {
    \textbf{Endogenous}\\
    \textbf{Variables}
};
\node[below=0.4cm of y4.south, align=center] (label) {$\hat{v}_i$};

% Arrows from scoring to predictions
\draw[arrowstyle] (f1) to [] (y1);
\draw[arrowstyle] (f2) to [] (y2);
\draw[arrowstyle] (f3) to [] (y3);
\draw[arrowstyle] (f4) to [] (y4);

\end{tikzpicture}
}



\newcommand{\CCEMtest}{
\begin{tikzpicture}[
    node distance = .3cm,
]

% Position
\node[square1] (sq41) {};
\node[square2] (sq42) [right=0cm of sq41] {};
\node[square3] (sq43) [right=0cm of sq42] {};
\node[above=0cm of sq42.north] (label) {Top};
\node[operation] (s4) [right= of sq43] {$s$};
\draw[arrowstyle] (sq43) to [] (s4);
\node[true] (c4) [right= of s4] {\cmark};
\draw[arrowstyle] (s4) to [] (c4);
\node[operation] (ceop4) [right= of c4] {$\omega$};
\draw[arrowstyle] (c4) to [] (ceop4);
\node[cembtrue1] (ce41) [right= of ceop4] {};
\node[cembtrue2] (ce42) [right=0cm of ce41] {};
\node[cembtrue3] (ce43) [right=0cm of ce42] {};
\node[above=0cm of ce42.north] (label) {Top};
\draw[arrowstyle] (ceop4) to [] (ce41);
\draw[arrowstyle] (sq42.south) -- ++(0,-0.4) -| (ceop4.south);

% Color
% \node[operation] (agg2) [below=.7cm of ce42] {$\oplus$};
% \node[square1] (cep21) [below= of agg2, xshift=-0.cm] {};
% \node[square3] (cep22) [right=0cm of cep21] {};
\node[operation] (f2) [below=.7cm of ce42] {$f_w$};
\node[left=0.1cm of f2.west, xshift=0.cm] (label) {White};
\draw[adjweightbig] (ce42) -- (f2) node[midway, right] {$a_{w,t}$};
% \draw[arrowstyle] (agg2) to [] (cep21);
% \draw[arrowstyle] (cep22) to [] (f2);
\node[false] (y2) [right= of f2] {\xmark};
\draw[arrowstyle] (f2) to [] (y2);
\node[operation] (ceop2) [right= of y2] {$\omega$};
\node[cembfalse1] (ce21) [right= of ceop2] {};
\node[cembfalse2] (ce22) [right=0cm of ce21] {};
\node[cembfalse3] (ce23) [right=0cm of ce22] {};
\node[above=0cm of ce22.north] (label) {White};
\draw[arrowstyle] (y2) to [] (ceop2);
\node[square2] (sq22) [above= of ceop2] {};
\node[square1] (sq21) [left=0cm of sq22] {};
\node[square3] (sq23) [right=0cm of sq22] {};
\node[above=0cm of sq22.north] (label) {White};
\draw[arrowstyle] (sq22) to [] (ceop2);
\draw[arrowstyle] (ceop2) to [] (ce21);

% Object
% \node[operation] (agg1) [below=.7cm of ce22] {$\oplus$};
% \node[square1] (cep11) [right= of agg1, xshift=-0.cm] {};
% \node[square3] (cep12) [right=0cm of cep11] {};
\node[operation] (f1) [below=.7cm of ce22] {$f_r$};
\draw[adjweightbig] (ce22) -- (f1) node[midway, right] {$a_{r,w}$};
% \draw[arrowstyle] (agg1) to [] (cep11);
% \draw[arrowstyle] (cep12) to [] (f1);
\node[true] (y1) [right= of f1] {\cmark};
\node[below=0.cm of y1.south, xshift=.2cm] (label) {RedHeart};
\draw[arrowstyle] (f1) to [] (y1);


% Shape
\node[cembfalse2] (ce32) [below=.7cm of f1] {};
\node[cembfalse1] (ce31) [left=0cm of ce32] {};
\node[cembfalse3] (ce33) [right=0cm of ce32] {};
\node[below=.cm of ce32.south] (label) {Square};
\draw[adjweightbig] (ce32) -- (f1) node[midway, left] {$a_{r,s}$};
\node[operation] (ceop3) [left= of ce31] {$\omega$};
\node[false] (c3) [left= of ceop3] {\xmark};
\node[operation] (s3) [left= of c3] {$s$};
\node[square3] (sq33) [left= of s3] {};
\node[square2] (sq32) [left=0cm of sq33] {};
\node[square1] (sq31) [left=0cm of sq32] {};
\node[left=.1cm of sq31.west] (label) {Square};
\draw[arrowstyle] (sq33) to [] (s3);
\draw[arrowstyle] (s3) to [] (c3);
\draw[arrowstyle] (c3) to [] (ceop3);
\draw[arrowstyle] (ceop3) to [] (ce31);
\draw[arrowstyle] (sq32.south) -- ++(0,-0.4) -| (ceop3.south);



\node[below= 2cm of sq43.center, inner sep=0pt] (img_dsprites) {\includegraphics[width=1cm]{figs/h_dsprites.png}};
\node[below=.cm of img_dsprites.south, align=center] (label) {
    \textbf{Input}
};
\draw[arrowstyledash] (img_dsprites) to [bend left=20] (sq41);
\draw[arrowstyledash] (img_dsprites) to [bend left=20] (sq31);
\draw[arrowstyledash] (img_dsprites) to [bend left=30] (sq21);


\end{tikzpicture}
}


\tikzset{
    % main node/.style = {circle, draw=none, thick, fill=gray!20},
    % message node/.style = {rectangle, draw=none, thick, fill=green!20, align=center},
    observed/.style={circle, draw, thick, fill=gray!50, minimum size=.7cm},
    unobserved/.style={circle, draw, thick, minimum size=.7cm},
    blank/.style={circle, draw, thick, dotted, minimum size=.7cm, opacity=0.5},
}
\newcommand{\ccempgm}{
\begin{tikzpicture}[
    node distance = .4cm,
]

\node[observed] (x) {$x$};
\node[unobserved] (u1) [right= of x, yshift=1.1cm] {$u_1$};
\node[unobserved] (u2) [below=.2cm of u1] {$u_2$};
\node[unobserved, draw=none, fill=none] (ui) [below=-.1cm of u2] {$\dots$};
\node[unobserved] (uk) [below=-.1cm of ui] {$u_k$};
\node[unobserved] (v1) [right= of u1] {$v_1$};
\node[unobserved] (v2) [right= of u2] {$v_2$};
\node[unobserved, draw=none, fill=none] (vi) [right= of ui] {$\dots$};
\node[unobserved] (vk) [right= of uk] {$v_k$};
\draw[arrowstyle] (x) -- (u1);
\draw[arrowstyle] (x) -- (u2);
\draw[arrowstyle] (x) -- (uk);
\draw[arrowstyle] (u1) -- (v1);
\draw[arrowstyle] (u2) -- (v2);
\draw[arrowstyle] (uk) -- (vk);
\draw[arrowstyle] (v1) to[bend left=60] (vk);
\draw[arrowstyle] (v1) to[bend left=30] (v2);
\draw[arrowstyle] (v2) to[bend left=30] (v1);
\draw[arrowstyle] (v2) to[bend left=30] (vk);
\draw[arrowstyle] (vk) to[bend right=80] (v1);
\draw[arrowstyle] (vk) to[bend left=30] (v2);

\end{tikzpicture}
}

\newcommand{\ccemcutset}{
\begin{tikzpicture}[
    node distance = .7cm,
]

\node[observed] (x) {$x$};
\node[unobserved] (u1) [right= of x, yshift=1.1cm] {$u_1$};
\node[unobserved] (u2) [below=.2cm of u1] {$u_2$};
\node[unobserved, draw=none, fill=none] (ui) [below=-.1cm of u2] {$\dots$};
\node[unobserved] (uk) [below=-.1cm of ui] {$u_k$};
\node[unobserved] (v1p) [right= of u1] {$v_1'$};
\node[unobserved] (v2p) [right= of u2] {$v_2'$};
\node[unobserved, draw=none, fill=none] (vip) [right= of ui] {$\dots$};
\node[unobserved] (vkp) [right= of uk] {$v_k'$};
\node[unobserved] (v1) [right= of v1p] {$v_1$};
\node[unobserved] (v2) [right= of v2p] {$v_2$};
\node[unobserved, draw=none, fill=none] (vi) [right= of vip] {$\dots$};
\node[unobserved] (vk) [right= of vkp] {$v_k$};
\draw[arrowstyle] (x) -- (u1);
\draw[arrowstyle] (x) -- (u2);
\draw[arrowstyle] (x) -- (uk);
\draw[arrowstyle] (u1) -- (v1p);
\draw[arrowstyle] (u2) -- (v2p);
\draw[arrowstyle] (uk) -- (vkp);
% \draw[arrowstyle] (v1p) -- (v1);
% \draw[arrowstyle] (v2p) -- (v2);
% \draw[arrowstyle] (vkp) -- (vk);
\draw[arrowstyle] (v1p) -- (v2);
\draw[arrowstyle] (v1p) -- (vk);
\draw[arrowstyle] (v2p) -- (v1);
\draw[arrowstyle] (v2p) -- (vk);
\draw[arrowstyle] (vkp) -- (v1);
\draw[arrowstyle] (vkp) -- (v2);
\draw[arrowstyle] (u1) to[bend left=30] (v1);
\draw[arrowstyle] (u2) to[bend right=30] (v2);
\draw[arrowstyle] (uk) to[bend right=30] (vk);

\end{tikzpicture}
}

\newcommand{\ccemcutsetxai}{
\begin{tikzpicture}[
    node distance = .7cm,
]

\node[observed] (x) {$x$};
\node[unobserved, draw=none, fill=none] (implies) [left=.0cm of x, yshift=.5cm] {\large{$roots(\mathcal{G}') = \{v_2'\}$}};
\node[unobserved, draw=none, fill=none] (implies2) [left=.0cm of x, yshift=-.5cm] {\large{$ch(roots(\mathcal{G}')) = \{v_k\}$}};
\node[unobserved] (u1) [right= of x, yshift=1.1cm] {$u_1$};
\node[unobserved] (u2) [below=.2cm of u1] {$u_2$};
\node[unobserved, draw=none, fill=none] (ui) [below=-.1cm of u2] {$\dots$};
\node[unobserved] (uk) [below=-.1cm of ui] {$u_k$};
\node[unobserved] (v1p) [right= of u1] {$v_1'$};
\node[unobserved] (v2p) [right= of u2] {$v_2'$};
\node[unobserved, draw=none, fill=none] (vip) [right= of ui] {$\dots$};
\node[unobserved] (vkp) [right= of uk] {$v_k'$};
\node[unobserved] (v1) [right= of v1p] {$v_1$};
\node[unobserved] (v2) [right= of v2p] {$v_2$};
\node[unobserved, draw=none, fill=none] (vi) [right= of vip] {$\dots$};
\node[unobserved] (vk) [right= of vkp] {$v_k$};
\draw[arrowstyle] (x) -- (u1);
\draw[arrowstyle] (x) -- (u2);
\draw[arrowstyle] (x) -- (uk);
\draw[arrowstyle] (u1) -- (v1p);
\draw[arrowstyle] (u2) -- (v2p);
\draw[arrowstyle] (uk) -- (vkp);
% \draw[arrowstyle] (v1p) -- (v1);
% \draw[arrowstyle] (v2p) -- (v2);
% \draw[arrowstyle] (vkp) -- (vk);
% \draw[arrowstyledash] (v1p) -- (v2);
% \draw[arrowstyledash] (v1p) -- (vk);
% \draw[arrowstyledash] (v2p) -- (v1);
\draw[adjweightbig] (v2p) -- (vk);
\draw[adjweightbig] (vkp) -- (v1);
% \draw[arrowstyledash] (vkp) -- (v2);
\draw[arrowstyle] (u1) to[bend left=30] (v1);
\draw[arrowstyle] (u2) to[bend right=30] (v2);
\draw[arrowstyle] (uk) to[bend right=30] (vk);

\node[observed] (x2) [right=6.0cm of x] {$x$};
\node[unobserved, draw=none, fill=none] (implies) [left=.0cm of x2, yshift=.0cm] {\Large{$\implies$}};
\node[unobserved] (u12) [right= of x2, yshift=1.1cm] {$u_1$};
\node[unobserved] (u22) [below=.2cm of u12] {$u_2$};
\node[unobserved, draw=none, fill=none] (ui2) [below=-.1cm of u22] {$\dots$};
\node[unobserved] (uk2) [below=-.1cm of ui2] {$u_k$};
\node[blank] (v1p2) [right= of u12] {$v_1'$};
\node[unobserved] (v2p2) [right= of u22] {$v_2'$};
\node[unobserved, draw=none, fill=none] (vip2) [right= of ui2] {$\dots$};
\node[blank] (vkp2) [right= of uk2] {$v_k'$};
\node[blank] (v12) [right= of v1p2] {$v_1$};
\node[blank] (v22) [right= of v2p2] {$v_2$};
\node[unobserved, draw=none, fill=none] (vi2) [right= of vip2] {$\dots$};
\node[unobserved] (vk2) [right= of vkp2] {$v_k$};
\node[unobserved] (v1s2) [right= of v12] {$v_1$};
\node[blank] (v2s2) [right= of v22] {$v_2$};
% \node[unobserved, draw=none, fill=none] (vis) [right= of vi] {$\dots$};
\node[blank] (vks2) [right= of vk2] {$v_k$};
\draw[arrowstyle] (x2) -- (u12);
\draw[arrowstyle] (x2) -- (u22);
\draw[arrowstyle] (x2) -- (uk2);
% \draw[arrowstyle] (u1) -- (v1p);
\draw[arrowstyle] (u22) -- (v2p2);
% \draw[arrowstyle] (uk) -- (vkp);
% \draw[arrowstyle] (v1p) -- (v1);
% \draw[arrowstyle] (v2p) -- (v2);
% \draw[arrowstyle] (vkp) -- (vk);
% \draw[arrowstyle] (v1p) -- (v2);
% \draw[arrowstyle] (v1p) -- (vk);
% \draw[arrowstyle] (v2p) -- (v1);
\draw[adjweightbig] (v2p2) -- (vk2);
\draw[adjweightbig] (vk2) -- (v1s2);
% \draw[arrowstyle] (vkp) -- (v2);
\draw[arrowstyle] (u12) to[bend left=30] (v1s2);
% \draw[arrowstyle] (u2) to[bend right=30] (v2);
\draw[arrowstyle] (uk2) to[bend right=30] (vk2);
\node[above=.4cm of vk2.east, xshift=1.3cm, yshift=.0cm, align=center, fill=white] (label) {
    \small{\textcolor{blue!50}{\textbf{explaining subgraph}}}
};

% \node[unobserved, draw=none, fill=none] (v1text) [above=-2.cm of implies.north] {\large{$p(v_1 \mid v_k', u_1; \theta_f) = p(v_1 \mid v_k, u_1; \theta_f)$}};

\end{tikzpicture}
}


\newcommand{\ccemcutsetunroll}{
\begin{tikzpicture}[
    node distance = .7cm,
]

\node[observed] (x) {$x$};
\node[unobserved, draw=none, fill=none] (implies) [left=.0cm of x, yshift=.0cm] {\Large{$\implies$}};
\node[unobserved] (u1) [right= of x, yshift=1.1cm] {$u_1$};
\node[unobserved] (u2) [below=.2cm of u1] {$u_2$};
\node[unobserved, draw=none, fill=none] (ui) [below=-.1cm of u2] {$\dots$};
\node[unobserved] (uk) [below=-.1cm of ui] {$u_k$};
\node[blank] (v1p) [right= of u1] {$v_1'$};
\node[unobserved] (v2p) [right= of u2] {$v_2'$};
\node[unobserved, draw=none, fill=none] (vip) [right= of ui] {$\dots$};
\node[blank] (vkp) [right= of uk] {$v_k'$};
\node[blank] (v1) [right= of v1p] {$v_1$};
\node[blank] (v2) [right= of v2p] {$v_2$};
\node[unobserved, draw=none, fill=none] (vi) [right= of vip] {$\dots$};
\node[unobserved] (vk) [right= of vkp] {$v_k$};
\node[unobserved] (v1s) [right= of v1] {$v_1$};
\node[blank] (v2s) [right= of v2] {$v_2$};
% \node[unobserved, draw=none, fill=none] (vis) [right= of vi] {$\dots$};
\node[blank] (vks) [right= of vk] {$v_k$};
\draw[arrowstyle] (x) -- (u1);
\draw[arrowstyle] (x) -- (u2);
\draw[arrowstyle] (x) -- (uk);
% \draw[arrowstyle] (u1) -- (v1p);
\draw[arrowstyle] (u2) -- (v2p);
% \draw[arrowstyle] (uk) -- (vkp);
% \draw[arrowstyle] (v1p) -- (v1);
% \draw[arrowstyle] (v2p) -- (v2);
% \draw[arrowstyle] (vkp) -- (vk);
% \draw[arrowstyle] (v1p) -- (v2);
% \draw[arrowstyle] (v1p) -- (vk);
% \draw[arrowstyle] (v2p) -- (v1);
\draw[adjweightbig] (v2p) -- (vk);
\draw[adjweightbig] (vk) -- (v1s);
% \draw[arrowstyle] (vkp) -- (v2);
\draw[arrowstyle] (u1) to[bend left=30] (v1s);
% \draw[arrowstyle] (u2) to[bend right=30] (v2);
\draw[arrowstyle] (uk) to[bend right=30] (vk);
\node[above=.4cm of vk.east, xshift=1.3cm, yshift=.0cm, align=center, fill=white] (label) {
    \small{\textcolor{blue!50}{\textbf{explaining subgraph}}}
};

\end{tikzpicture}
}



\newcommand{\scm}{
\begin{tikzpicture}[
    node distance = .4cm,
]

\node[true] (v1) [] {$v_1$};
\node[true] (v2) [below= of v1] {$v_2$};
\node[true] (v3) [right= of v2] {$v_3$};
\node[false] (v4) [right= of v1] {$v_4$};
\node[true] (v5) [right= of v4] {$v_5$};

\draw[arrowstyle] (v1) -- (v2);
\draw[arrowstyle] (v2) -- (v3);
% \draw[arrowstyle] (v3) -- (v4);
% \draw[arrowstyle] (v1) -- (v4);
\draw[arrowstyle] (v4) -- (v5);
\draw[arrowstyle] (v3) -- (v5);

\begin{pgfonlayer}{background}
\draw[->, dashed, thick, gray] ([yshift=1mm]v2.south) -- ([yshift=1mm, xshift=1mm]v3.south) -- ([yshift=-2mm, xshift=-2mm]v5.south);
\end{pgfonlayer}

\node[below=.0cm of v2.south, xshift=.6cm, color=gray] (label) {effect path};
    
\end{tikzpicture}
}

\newcommand{\scmdo}{
\begin{tikzpicture}[
    node distance = .4cm,
]

\node[true] (v1) [] {$v_1$};
\node[true] (v2) [below= of v1] {$v_2$};
\node[true] (v3) [right= of v2] {$v_3$};
\node[false] (v4) [right= of v1] {$v_4$};
\node[true] (v5) [right= of v4] {$v_5$};

% \draw[arrowstyle] (v1) -- (v2);
\draw[arrowstyle] (v2) -- (v3);
% \draw[arrowstyle] (v3) -- (v4);
\draw[arrowstyle] (v3) -- (v5);
% \draw[arrowstyle] (v1) -- (v4);
\draw[arrowstyle] (v4) -- (v5);


\begin{pgfonlayer}{background}
\draw[->, dashed, thick, gray] ([yshift=1mm]v2.south) -- ([yshift=1mm, xshift=1mm]v3.south) -- ([yshift=-2mm, xshift=-2mm]v5.south);
\end{pgfonlayer}

\node[right=0cm of v3.east, yshift=-3mm, xshift=-3mm, gray] (label) {$\hat{v}_3=v_3$};
\node[below=0cm of v2.south] (label) {do$(v_2=1)$};
    
\end{tikzpicture}
}


\newcommand{\scmgt}{
\begin{tikzpicture}[
    node distance = .4cm,
]

\node[true] (v1) [] {$v_1$};
\node[true] (v2) [below= of v1] {$v_2$};
\node[false] (v3) [right= of v2] {$v_3$};
\node[false] (v4) [right= of v1] {$v_4$};
\node[false] (v5) [right= of v4] {$v_5$};

\draw[arrowstyle] (v1) -- (v2);
\draw[arrowstyle] (v2) -- (v3);
% \draw[arrowstyle] (v3) -- (v4);
\draw[arrowstyle] (v3) -- (v5);
% \draw[arrowstyle] (v1) -- (v4);
\draw[arrowstyle] (v4) -- (v5);


\begin{pgfonlayer}{background}
\draw[->, dashed, thick, gray] ([yshift=1mm]v2.south) -- ([yshift=1mm, xshift=1mm]v3.south) -- ([yshift=-2mm, xshift=-2mm]v5.south);
\end{pgfonlayer}

\node[right=0cm of v3.east, yshift=-3mm] (label) {$\hat{v}_3=v_3$};
    
\end{tikzpicture}
}


\newcommand{\scmblock}{
\begin{tikzpicture}[
    node distance = .4cm,
]
\node[true] (v1) [] {$v_1$};
\node[false] (v2) [below= of v1] {$v_2$};
\node[true] (v3) [right= of v2] {$v_3$};
\node[false] (v4) [right= of v1] {$v_4$};
\node[true] (v5) [right= of v4] {$v_5$};

% \draw[arrowstyle] (v2) -- (v3);
% \draw[arrowstyle] (v3) -- (v4);
\draw[arrowstyle] (v3) -- (v5);
% \draw[arrowstyle] (v1) -- (v4);
\draw[arrowstyle] (v4) -- (v5);

\begin{pgfonlayer}{background}
\draw[-|, dashed, thick, gray] ([yshift=1mm]v2.south) -- ([yshift=1mm, xshift=-4mm]v3.south);
\end{pgfonlayer}

\node[below=0cm of v2.south] (label) {do$(v_2=0)$};
\node[right=0cm of v3.east] (label) {do$(v_3=1)$};
\end{tikzpicture}
}

\tikzset{
    inarrows/.style={->, rounded corners, dash pattern=on 2pt off .6pt, gray},
    true2/.style = {circle, draw=none, thick, fill=orange!30, minimum width=.5cm, minimum height=.5cm, inner sep=0pt},
    false2/.style = {circle, draw=none, thick, fill=violet!30, minimum width=.5cm, minimum height=.5cm, inner sep=0pt},
    nocause/.style={-, rounded corners, dash pattern=on 2pt off .6pt, gray},
}
\newcommand{\cm}{
\begin{tikzpicture}[
    node distance = .2cm,
]

% \node[inner sep=0pt] (img_dsprites) {\includegraphics[width=.8cm]{figs/h_dsprites.png}};
% \node[below=0cm of img_dsprites.south, align=center] (label) {
%     \tiny{\textbf{Input}}
% };

\node[true2] (vd) [above= of g] {$v_d$};
\node[true2] (vy) [left=1.1cm of vd, yshift=-.3cm] {$v_y$};
\node[true2] (vx) [right=1.1cm of vd, yshift=-.3cm] {$v_x$};
\node[true2] (vc) [above= of vy] {$v_c$};
\node[true2] (vs) [above= of vx] {$v_s$};
\node[false2] (vo) [above=.5 of vd] {$v_o$};

\node[right=0.cm of vo.east, align=center, color=violet!50] (label) {
    \small{\textbf{Target}}
};
% \node[below=-0.08cm of fo.south, align=center, color=blue!50] (label) {
%     \tiny{\textbf{Class}}
% };
% \node[below=.1cm of fo.south, align=center, color=blue!50] (label) {
%     \tiny{\textbf{Predictors}}
% };

% \node[above=0.1cm of vs.north, align=center, color=green!70!black] (label) {
%     \tiny{\textbf{Interpretable}}
% };
% \node[above=-0.08cm of vs.north, align=center, color=green!70!black] (label) {
%     \tiny{\textbf{Variables}}
% };

\draw[arrowstyle] (vx) -- (vs);
\draw[arrowstyle] (vy) -- (vc);
% \draw[arrowstyle] (vd) -- (fc);
\draw[arrowstyle] (vd) -- (vc);
\draw[arrowstyle] (vc) -- (vo);
\draw[arrowstyle] (vs) -- (vo);
% \draw[arrowstyle] (v3) -- (v4);
% \draw[arrowstyle] (v3) -- (v5);
% \draw[arrowstyle] (v1) -- (v4);
% \draw[arrowstyle] (v4) -- (v5);

% \begin{pgfonlayer}{background}
% \draw[-|, dashed, thick, gray] ([yshift=1mm]v2.south) -- ([yshift=1mm, xshift=-4mm]v3.south);
% \end{pgfonlayer}

% \node[below=0cm of v2.south] (label) {do$(v_2=0)$};
% \node[right=0cm of v3.east] (label) {do$(v_3=1)$};
\end{tikzpicture}
}

\newcommand{\vizabs}{
\begin{tikzpicture}[
    node distance = .2cm,
]

% \node[inner sep=0pt] (img_dsprites) {\includegraphics[width=.8cm]{figs/h_dsprites.png}};
% \node[below=0cm of img_dsprites.south, align=center] (label) {
%     \tiny{\textbf{Input}}
% };

\node[plain] (x1) [] {$x_1$};
\node[plain] (x2) [right= of x1] {$x_2$};
\node[plain] (x3) [right= of x2] {$x_3$};
\node[plain] (xi) [right= of x3] {$\dots$};
\node[plain] (xd) [right= of xi] {$x_d$};
\node[below=0cm of x3.south, align=center] (label) {
    \small{\textbf{Raw Features}}
};

\node[operation] (g) [above= of x3] {$g$};

\node[true2] (vd) [above= of g] {$v_d$};
\node[true2] (vy) [left=1.1cm of vd, yshift=-.3cm] {$v_y$};
\node[true2] (vx) [right=1.1cm of vd, yshift=-.3cm] {$v_x$};
\node[operation] (fc) [above= of vy] {$f_c$};
\node[operation] (fs) [above= of vx] {$f_s$};
\node[true2] (vc) [above= of fc] {$v_c$};
\node[operation] (fo) [right=1.1cm of vc] {$f_o$};
\node[true2] (vs) [above= of fs] {$v_s$};
\node[false2] (vo) [above= of fo] {$v_o$};

\node[right=0.cm of vo.east, align=center, color=violet!50] (label) {
    \small{\textbf{Target}}
};
% \node[below=-0.08cm of fo.south, align=center, color=blue!50] (label) {
%     \tiny{\textbf{Class}}
% };
% \node[below=.1cm of fo.south, align=center, color=blue!50] (label) {
%     \tiny{\textbf{Predictors}}
% };

% \node[above=0.1cm of vs.north, align=center, color=green!70!black] (label) {
%     \tiny{\textbf{Interpretable}}
% };
% \node[above=-0.08cm of vs.north, align=center, color=green!70!black] (label) {
%     \tiny{\textbf{Variables}}
% };

\draw[nocause] (x1) to (g);
\draw[nocause] (x2) to (g);
\draw[nocause] (x3) to (g);
\draw[nocause] (xi) to (g);
\draw[nocause] (xd) to (g);
\draw[nocause] (g) to[bend left=20] (vy);
\draw[nocause] (g) to[bend right=5] (vc);
\draw[nocause] (g) to[bend right=0] (vd);
\draw[nocause] (g) to[bend left=5] (vs);
\draw[nocause] (g) to[bend right=20] (vx);
\draw[arrowstyle] (vx) -- (fs);
\draw[arrowstyle] (vy) -- (fc);
\draw[arrowstyle] (vx) -- (fo);
\draw[arrowstyle] (fc) -- (vc);
\draw[arrowstyle] (fs) -- (vs);
% \draw[arrowstyle] (vd) -- (fc);
\draw[arrowstyle] (vd) -- (fc);
\draw[arrowstyle] (vc) -- (fo);
\draw[arrowstyle] (vs) -- (fo);
\draw[arrowstyle] (fo) -- (vo);
% \draw[arrowstyle] (v3) -- (v4);
% \draw[arrowstyle] (v3) -- (v5);
% \draw[arrowstyle] (v1) -- (v4);
% \draw[arrowstyle] (v4) -- (v5);

% \begin{pgfonlayer}{background}
% \draw[-|, dashed, thick, gray] ([yshift=1mm]v2.south) -- ([yshift=1mm, xshift=-4mm]v3.south);
% \end{pgfonlayer}

% \node[below=0cm of v2.south] (label) {do$(v_2=0)$};
% \node[right=0cm of v3.east] (label) {do$(v_3=1)$};
\end{tikzpicture}
}


\newcommand{\vizabsfull}{
\begin{tikzpicture}[
    node distance = .2cm,
]

% \node[inner sep=0pt] (img_dsprites) {\includegraphics[width=.8cm]{figs/h_dsprites.png}};
% \node[below=0cm of img_dsprites.south, align=center] (label) {
%     \tiny{\textbf{Input}}
% };

\node[plain] (x1) [] {$x_1$};
\node[plain] (x2) [right= of x1] {$x_2$};
\node[plain] (x3) [right= of x2] {$x_3$};
\node[plain] (xi) [right= of x3] {$\dots$};
\node[plain] (xd) [right= of xi] {$x_d$};
\node[below=0cm of x3.south, align=center] (label) {
    \small{\textbf{Raw Features}}
};

\node[operation] (g) [above= of x3] {$g$};

\node[true2] (vd) [above=.3cm of g] {$v_d$};
\node[operation] (fd) [above=.5cm of vd] {$f_d$};
\node[true2] (vy) [left= of vd] {$v_y$};
\node[operation] (fy) [above=.5cm of vy] {$f_y$};
\node[true2] (vx) [right= of vd] {$v_x$};
\node[operation] (fx) [above=.5cm of vx] {$f_x$};
\node[true2] (vc) [right= of vx] {$v_c$};
\node[operation] (fc) [above=.5cm of vc] {$f_c$};
\node[true2] (vs) [left= of vy] {$v_s$};
\node[operation] (fs) [above=.5cm of vs] {$f_s$};
\node[operation] (fo) [right= of fc] {$f_o$};
\node[true2] (vdp) [above=.3cm of fd] {$v_d^'$};
\node[true2] (vyp) [above=.3cm of fy] {$v_y^'$};
\node[true2] (vxp) [above=.3cm of fx] {$v_x^'$};
\node[true2] (vcp) [above=.3cm of fc] {$v_c^'$};
\node[true2] (vsp) [above=.3cm of fs] {$v_s^'$};
\node[false2] (vop) [above=.3cm of fo] {$v_o$};



\node[above=0.23cm of vsp.north, align=center, color=orange!70] (label) {
    \small{\textbf{High-Level}}
};
\node[above=-0.08cm of vsp.north, align=center, color=orange!70] (label) {
    \small{\textbf{Concepts}}
};

\node[below=-0.08cm of vs.south, align=center, color=orange!70] (label) {
    \small{\textbf{Concepts}}
};
\node[below=0.23cm of vs.south, align=center, color=orange!70] (label) {
    \small{\textbf{Copies}}
};
\node[above=0.0cm of vop.north, align=center, color=violet!50] (label) {
    \small{\textbf{Target}}
};


\draw[arrowstyle] (vd) to (fy);
\draw[arrowstyle] (vd) to (fx);
\draw[arrowstyle] (vd) to (fs);
\draw[arrowstyle] (vd) to (fc);

\draw[arrowstyle] (vy) to (fd);
\draw[arrowstyle] (vy) to (fx);
\draw[arrowstyle] (vy) to (fs);
\draw[arrowstyle] (vy) to (fc);

\draw[arrowstyle] (vx) to (fd);
\draw[arrowstyle] (vx) to (fy);
\draw[arrowstyle] (vx) to (fs);
\draw[arrowstyle] (vx) to (fc);

\draw[arrowstyle] (vs) to (fd);
\draw[arrowstyle] (vs) to (fy);
\draw[arrowstyle] (vs) to (fx);
\draw[arrowstyle] (vs) to (fc);

\draw[arrowstyle] (vc) to (fd);
\draw[arrowstyle] (vc) to (fy);
\draw[arrowstyle] (vc) to (fx);
\draw[arrowstyle] (vc) to (fs);

\draw[arrowstyle] (vd) to (fo);
\draw[arrowstyle] (vy) to (fo);
\draw[arrowstyle] (vx) to (fo);
\draw[arrowstyle] (vs) to (fo);
\draw[arrowstyle] (vc) to (fo);

\draw[arrowstyle] (fd) to (vdp);
\draw[arrowstyle] (fy) to (vyp);
\draw[arrowstyle] (fx) to (vxp);
\draw[arrowstyle] (fs) to (vsp);
\draw[arrowstyle] (fc) to (vcp);

\draw[arrowstyle] (fo) to (vop);
\draw[nocause] (x1) to (g);
\draw[nocause] (x2) to (g);
\draw[nocause] (x3) to (g);
\draw[nocause] (xi) to (g);
\draw[nocause] (xd) to (g);
\draw[nocause] (g) to (vd);
\draw[nocause] (g) to (vy);
\draw[nocause] (g) to (vx);
\draw[nocause] (g) to (vs);
\draw[nocause] (g) to (vc);

% \begin{pgfonlayer}{background}
% \draw[-|, dashed, thick, gray] ([yshift=1mm]v2.south) -- ([yshift=1mm, xshift=-4mm]v3.south);
% \end{pgfonlayer}

% \node[below=0cm of v2.south] (label) {do$(v_2=0)$};
% \node[right=0cm of v3.east] (label) {do$(v_3=1)$};
\end{tikzpicture}
}

\newcommand{\vizabssparse}{
\begin{tikzpicture}[
    node distance = .2cm,
]

% \node[inner sep=0pt] (img_dsprites) {\includegraphics[width=.8cm]{figs/h_dsprites.png}};
% \node[below=0cm of img_dsprites.south, align=center] (label) {
%     \tiny{\textbf{Input}}
% };

\node[plain] (x1) [] {$x_1$};
\node[plain] (x2) [right= of x1] {$x_2$};
\node[plain] (x3) [right= of x2] {$x_3$};
\node[plain] (xi) [right= of x3] {$\dots$};
\node[plain] (xd) [right= of xi] {$x_d$};
\node[below=0cm of x3.south, align=center] (label) {
    \small{\textbf{Raw Features}}
};

\node[operation] (g) [above= of x3] {$g$};

\node[true2] (vd) [above=.3cm of g] {$v_d$};
\node[operation, opacity=0.2] (fd) [above=.5cm of vd] {$f_d$};
\node[true2] (vy) [left= of vd] {$v_y$};
\node[operation, opacity=0.2] (fy) [above=.5cm of vy] {$f_y$};
\node[true2] (vx) [right= of vd] {$v_x$};
\node[operation, opacity=0.2] (fx) [above=.5cm of vx] {$f_x$};
\node[true2] (vc) [right= of vx] {$v_c$};
\node[operation] (fc) [above=.5cm of vc] {$f_c$};
\node[true2] (vs) [left= of vy] {$v_s$};
\node[operation] (fs) [above=.5cm of vs] {$f_s$};
\node[operation] (fo) [right= of fc] {$f_o$};
\node[true2, opacity=0.2] (vdp) [above=.3cm of fd] {$v_d^'$};
\node[true2, opacity=0.2] (vyp) [above=.3cm of fy] {$v_y^'$};
\node[true2, opacity=0.2] (vxp) [above=.3cm of fx] {$v_x^'$};
\node[true2] (vcp) [above=.3cm of fc] {$v_c^'$};
\node[true2] (vsp) [above=.3cm of fs] {$v_s^'$};
\node[false2] (vop) [above=.3cm of fo] {$v_o$};



\node[above=0.23cm of vsp.north, align=center, color=orange!70] (label) {
    \small{\textbf{High-Level}}
};
\node[above=-0.08cm of vsp.north, align=center, color=orange!70] (label) {
    \small{\textbf{Concepts}}
};

\node[below=-0.08cm of vs.south, align=center, color=orange!70] (label) {
    \small{\textbf{Concepts}}
};
\node[below=0.23cm of vs.south, align=center, color=orange!70] (label) {
    \small{\textbf{Copies}}
};
\node[above=0.0cm of vop.north, align=center, color=violet!50] (label) {
    \small{\textbf{Target}}
};



\draw[arrowstyle] (vd) to (fc);

\draw[arrowstyle] (vy) to (fc);

\draw[arrowstyle] (vx) to (fs);

\draw[arrowstyle] (vs) to (fo);
\draw[arrowstyle] (vc) to (fo);

\draw[arrowstyle, opacity=0.2] (fd) to (vdp);
\draw[arrowstyle, opacity=0.2] (fy) to (vyp);
\draw[arrowstyle, opacity=0.2] (fx) to (vxp);
\draw[arrowstyle] (fs) to (vsp);
\draw[arrowstyle] (fc) to (vcp);

\draw[arrowstyle] (fo) to (vop);
\draw[nocause] (x1) to (g);
\draw[nocause] (x2) to (g);
\draw[nocause] (x3) to (g);
\draw[nocause] (xi) to (g);
\draw[nocause] (xd) to (g);
\draw[nocause] (g) to (vd);
\draw[nocause] (g) to (vy);
\draw[nocause] (g) to (vx);
\draw[nocause] (g) to (vs);
\draw[nocause] (g) to (vc);

% \begin{pgfonlayer}{background}
% \draw[-|, dashed, thick, gray] ([yshift=1mm]v2.south) -- ([yshift=1mm, xshift=-4mm]v3.south);
% \end{pgfonlayer}

% \node[below=0cm of v2.south] (label) {do$(v_2=0)$};
% \node[right=0cm of v3.east] (label) {do$(v_3=1)$};
\end{tikzpicture}
}


\newcommand{\blackbox}{
\begin{tikzpicture}[
    node distance = .2cm,
]

% \node[inner sep=0pt] (img_dsprites) {\includegraphics[width=.8cm]{figs/h_dsprites.png}};
\node[plain] (x1) [] {$x_1$};
\node[plain] (x2) [right= of x1] {$x_2$};
\node[plain] (x3) [right= of x2] {$x_3$};
\node[plain] (xi) [right= of x3] {$\dots$};
\node[plain] (xd) [right= of xi] {$x_d$};
\node[below=0cm of x3.south, align=center] (label) {
    \small{\textbf{Raw Features}}
};

\node[operation] (g) [above=.8cm of x3] {  Black Box  };
% \node[false] (vd) [above=1cm of img_dsprites, xshift=.3cm] {$v_d$};
% \node[false] (vy) [left= of vd] {$v_y$};
% \node[true] (vx) [right= of vd] {$v_x$};
% \node[true] (vc) [right= of vx] {$v_c$};
% \node[true] (vs) [left= of vy] {$v_s$};
\node[false2] (vo) [above=.8 of g] {$v_o$};

\node[right=0.cm of vo.east, align=center, color=violet!50] (label) {
    \small{\textbf{Target}}
};

\draw[nocause] (x1) to (g);
\draw[nocause] (x2) to (g);
\draw[nocause] (x3) to (g);
\draw[nocause] (xi) to (g);
\draw[nocause] (xd) to (g);
\draw[arrowstyle] (g) to (vo);

\end{tikzpicture}
}


\newcommand{\cf}{
\begin{tikzpicture}[
    node distance = .2cm,
]

% \node[inner sep=0pt] (img_dsprites) {\includegraphics[width=.8cm]{figs/h_dsprites.png}};
% \node[below=0cm of img_dsprites.south, align=center] (label) {
%     \tiny{\textbf{Input}}
% };

\node[plain] (x1) [] {$x_1$};
\node[plain] (x2) [right= of x1] {$x_2$};
\node[plain] (x3) [right= of x2] {$x_3$};
\node[plain] (xi) [right= of x3] {$\dots$};
\node[plain] (xd) [right= of xi] {$x_d$};
\node[below=0cm of x3.south, align=center] (label) {
    \small{\textbf{Raw Features}}
};

\node[false2] (vo) [above=2.3 of x3] {$v_o$};

% \node[above=0.1cm of vs.north, align=center, color=green!70!black] (label) {
%     \tiny{\textbf{Interpretable}}
% };
% \node[above=-0.08cm of vs.north, align=center, color=green!70!black] (label) {
%     \tiny{\textbf{Concepts}}
% };
% \node[right=0.cm of vo.east, align=center] (label) {
%     \tiny{\textbf{Task Label}}
% };

\draw[arrowstyle] (x1) to (vo);
\draw[arrowstyle] (x2) to (vo);
\draw[arrowstyle] (x3) to (vo);
\draw[arrowstyle] (xi) to (vo);
\draw[arrowstyle] (xd) to (vo);
% \draw[inarrows] (img_dsprites) to (vy);
% \draw[inarrows] (img_dsprites) to (vd);
% \draw[inarrows] (img_dsprites) to (vs);
% \draw[inarrows] (img_dsprites) to (vx);
% \draw[inarrows] (img_dsprites) to node[midway, fill=none, yshift=-.4cm, xshift=.1cm] {\tiny{\textbf{Encoders}}} (vc);

\end{tikzpicture}
}


\newcommand{\cbms}{
\begin{tikzpicture}[
    node distance = .2cm,
]

% \node[inner sep=0pt] (img_dsprites) {\includegraphics[width=.8cm]{figs/h_dsprites.png}};
% \node[below=0cm of img_dsprites.south, align=center] (label) {
%     \tiny{\textbf{Input}}
% };

\node[plain] (x1) [] {$x_1$};
\node[plain] (x2) [right= of x1] {$x_2$};
\node[plain] (x3) [right= of x2] {$x_3$};
\node[plain] (xi) [right= of x3] {$\dots$};
\node[plain] (xd) [right= of xi] {$x_d$};
\node[below=0cm of x3.south, align=center] (label) {
    \small{\textbf{Raw Features}}
};

\node[operation] (g) [above=.3cm of x3] {$g$};

\node[true2] (vd) [above=.3cm of g] {$v_d$};
\node[true2] (vy) [left= of vd] {$v_y$};
\node[true2] (vx) [right= of vd] {$v_x$};
\node[true2] (vc) [right= of vx] {$v_c$};
\node[true2] (vs) [left= of vy] {$v_s$};
\node[operation] (fo) [above=.3cm of vd] {$f_o$};
\node[false2] (vo) [above=.4cm of fo] {$v_o$};


\node[above=0.23cm of vs.north, align=center, color=orange!70] (label) {
    \small{\textbf{High-Level}}
};
\node[above=-0.08cm of vs.north, align=center, color=orange!70] (label) {
    \small{\textbf{Concepts}}
};
\node[right=0.cm of vo.east, align=center, color=violet!50] (label) {
    \small{\textbf{Target}}
};

\draw[arrowstyle] (vd) to (fo);
\draw[arrowstyle] (vy) to (fo);
\draw[arrowstyle] (vx) to (fo);
\draw[arrowstyle] (vs) to (fo);
\draw[arrowstyle] (vc) to (fo);
\draw[arrowstyle] (fo) to (vo);
\draw[nocause] (x1) to (g);
\draw[nocause] (x2) to (g);
\draw[nocause] (x3) to (g);
\draw[nocause] (xi) to (g);
\draw[nocause] (xd) to (g);
\draw[nocause] (g) to (vd);
\draw[nocause] (g) to (vy);
\draw[nocause] (g) to (vx);
\draw[nocause] (g) to (vs);
\draw[nocause] (g) to (vc);
% \draw[inarrows] (img_dsprites) to (vy);
% \draw[inarrows] (img_dsprites) to (vd);
% \draw[inarrows] (img_dsprites) to (vs);
% \draw[inarrows] (img_dsprites) to (vx);
% \draw[inarrows] (img_dsprites) to node[midway, fill=none, yshift=-.4cm, xshift=.1cm] {\tiny{\textbf{Encoders}}} (vc);

\end{tikzpicture}
}


\newcommand{\causalml}{
\begin{tikzpicture}[
    node distance = .3cm,
]

\node[true2] (vd) [] {$v_d$};
\node[true2] (vy) [left=.7cm of vd, yshift=-.3cm] {$v_y$};
\node[true2] (vx) [right=.7cm of vd, yshift=-.3cm] {$v_x$};
\node[operation] (fc) [above= of vy] {$f_c$};
\node[operation] (fs) [above= of vx] {$f_s$};
\node[true2] (vc) [above= of fc] {$v_c$};
\node[operation] (fo) [right=.7cm of vc] {$f_o$};
\node[true2] (vs) [above= of fs] {$v_s$};
\node[false2] (vo) [above= of fo] {$v_o$};

% \node[above=0.1cm of vs.north, align=center, color=green!70!black] (label) {
%     \tiny{\textbf{Interpretable}}
% };
% \node[above=-0.08cm of vs.north, align=center, color=green!70!black] (label) {
%     \tiny{\textbf{Variables}}
% };

\draw[arrowstyle] (vx) -- (fs);
\draw[arrowstyle] (vy) -- (fc);
\draw[arrowstyle] (fc) -- (vc);
\draw[arrowstyle] (fs) -- (vs);
\draw[arrowstyle] (vd) -- (fo);
\draw[arrowstyle] (vd) -- (fs);
\draw[arrowstyle] (vc) -- (fo);
\draw[arrowstyle] (vs) -- (fo);
\draw[arrowstyle] (fo) -- (vo);

\end{tikzpicture}
}


\newcommand{\genVSinfer}{
\begin{tikzpicture}[
    node distance = .3cm,
]

\node[plain] (x) [] {$x$};
\node[below=0cm of x.south, align=center] (label) {
    \small{\textbf{Raw Features}}
};

\node[false2] (vo) [above=1.5 of x] {$v_o$};
\node[above=0.08cm of vo.north, align=center, color=violet!50] (label) {
    \small{\textbf{Target}}
};


\draw[arrowstyle] (x) to[bend right=50] (vo);
\draw[arrowstyle] (vo) to[bend right=50] (x);

\node[above=.4cm of x.north, xshift=-.7cm, align=center, fill=white] (label) {
    \tiny{\textbf{Data Generation}}
};
\node[above=.1cm of x.north, xshift=-.7cm, align=center, fill=white] (label) {
    \tiny{\textbf{(Causal Discovery)}}
};
\node[above=1.cm of x.north, xshift=.7cm, align=center, fill=white] (label) {
    \tiny{\textbf{Model Inference}}
};
\node[above=.7cm of x.north, xshift=.7cm, align=center, fill=white] (label) {
    \tiny{\textbf{(Causal Opacity)}}
};


\end{tikzpicture}
}


\newcommand{\CausalStructure}{
\begin{tikzpicture}[scale=1]
%\node[color=black] (x1)  at (0,0) {\tiny $X_1$};
\node[color=black] (x1)  at (0,0) {Age};
\node[color=black] (x2)  at (4,0) {Income};
\node[color=black] (x3)  at (2,-2) {Risk of Hearth Attack};
%\draw[{Circle[open]}->] (x1) -- (x2);
%\draw[{Circle[open]}->] (x3) -- (x2);
\draw[->] (x1) -- (x3);
\draw[->] (x2) -- (x3);
\end{tikzpicture}
}


\newcommand{\CausalStructureTwo}{
\begin{tikzpicture}[scale=1]
%\node[color=black] (x1)  at (0,0) {\tiny $X_1$};
\node[color=black] (x1)  at (0,0) {Age};
\node[color=black] (x2)  at (4,0) {Income};
\node[color=black] (x3)  at (2,-2) {Risk of Hearth Attack};
\node[color=black] (x4)  at (4,2) {Gender};
%\draw[{Circle[open]}->] (x1) -- (x2);
%\draw[{Circle[open]}->] (x3) -- (x2);
\draw[->] (x1) -- (x3);
\draw[->] (x2) -- (x3);
\draw[->] (x4) -- (x2);
\end{tikzpicture}
}









==> long_intro_for_long_paper.tex <==

Deep Learning (DL) models have a pervasive impact on many areas of contemporary research and society \cite{Baldi2021}. 
Despite this success, there is growing concern about the widespread application of DL in society, particularly in ethically sensitive domains \citep{Dignum2019}. 
These concerns are partly due to the lack of \emph{causal explainability} of these models, which undermine their robustness, fairness and generalisability \cite{Scholkopf2021}.
Despite the use of a single term, the expression ``causal explainability'' can refer to two different, albeit related, problems \citep{Termine2023Causal}. 
One is the problem of \emph{causal opacity}, which denotes the difficulty of users to grasp and understand the ``hidden'' \emph{causal structure} characterising a model's inference and behaviour \citep{Termine2023Causal}.
The other is the problem of \emph{causal discovery}\footnote{\citet{Termine2023Causal} uses the term ``causal interpretability'' to denote this issue.} and concerns the possibility to use a model for detecting and understanding the \emph{causal mechanisms} beyond the regularities one can observe in data. 

Both problems can be better understood in the light of Pearl's account of causality \citep{Pearl2009, Pearl2019}, which measures an agent's causal understanding in terms of their ability to answer \emph{what-if} type of questions, and specifically \emph{interventional}  and \emph{counterfactual} questions (i.e., ``what if I do $X=x$?'' and ``what if I had observed $X=x^\prime$ instead of $X=x$?'', respectively). 
In this regard, causal opacity depends on the ability of users to answer interventional and counterfactual questions regarding the structure of a model's inference (e.g., what happens if I fix the feature \emph{age} to a value greater than $50$ instead of lower?).
This ability is fundamental to analysing the reliability and robustness of a model, and also plays an essential role in the task of verifying whether a model is \emph{fair}, especially within the now popular framework of \emph{counterfactual fairness} \citep{Kusner2017}.
%This form of causal understanding plays a central role in various domains of contemporary Artificial Intelligence (AI) research, in particular within the development and deployment of \emph{trustworthy} and \emph{explainable} AI systems \cite{Adadi2018, Minh2022, Beckers2022}.
%Indeed, intervention and counterfactual analyses are crucial 
%for control tasks and to analyse the reliability and robustness of a model, and plays an essential role also in the task of verifying whether a model is \emph{fair}, especially within the nowadays popular framework of \emph{counterfactual fairness} \citep{Kusner2017}.
For example, consider a recommendation system used by a financial institution to
to decide whether to give a loan to a particular customer.
One way to ensure the fairness of this system is to verify that sensitive attributes related to demographic groups, such as \emph{gender} or \emph{ethnicity}, have no causal relevance for the model's decision.
Such a verification task can be solved by checking that the model's predictions are robust (i.e., do not change) under interventional and counterfactual variations that affect sensitive attributes,
%That is, it ultimately involves the calculation of interventional and counterfactual questions, such as 
e.g., ``what will the model's decision be if I change the concept \emph{gender} from male to non-binary?''.

Causal opacity should be kept distinct from the problem of causal discovery, which instead depends on the (im)possibility of using DL models, and machine learning models more in general, to answer interventional and counterfactual questions that concern the hidden causal structure of the world.
This problem has been extensively analysed in causality literature \citep{Pearl2018, Pearl2019, Scholkopf2021} and notoriously depends on the pure ``associative'' nature of DL models, which allow them to make accurate predictions only within \emph{independent and identically distributed data}, whereas the computation of interventional and counterfactual questions require the ability to manage distribution shifts (e.g., induced by an intervention) and analyse out-of-distribution scenarios. 
Several techniques have been developed to discover causal mechanisms beyond data in the last years, especially in the domain of \emph{Causal Machine Learning} \citep{kaddour2022causal}.
In the present article, however, we are more concerned with methods and techniques  
%identifying and modelling the causal mechanisms generating the regularities one can observe in data.
%This problem and its implications for machine learning have been extensively discussed in causality literature  and and represents the main focus of the \emph{causal machine learning} research programme \citep{kaddour2022causal}.
%Although related, the problem causal discovery and the problem of causal opacity are concerned with two distinct kinds of causal understanding. Indeed, while the former focuses on understanding the causal structure \emph{of the world}, the latter focuses on understanding the causal structure \emph{of a model's inference}, i.e., on understanding the ``hidden'' network of causal implications that connect the various high-level concepts in a DL model's latent space and determine its observable predictive behaviour
%\textcolor{red}{(see, Fig. ***)}.
%This form of causal understanding plays a central role in various domains of contemporary Artificial Intelligence (AI) research, in particular within the development and deployment of \emph{trustworthy} and \emph{explainable} AI systems \cite{Adadi2018, Minh2022, Beckers2022}.
%Indeed, intervention and counterfactual analyses are crucial for control tasks and for verifying the reliability and robustness of DL models.
%Furthermore, these analysis are essential to verify whether a model is \emph{fair}, especially within the nowadays popular framework of \emph{counterfactual fairness} \citep{Kusner2017}.
%For example, consider a recommendation system used by a financial institution to
%to decide whether to give a loan to a particular customer.
%One way to ensure the fairness of this system is to verify that sensitive attributes related to demographic groups, such as \emph{gender} or \emph{ethnicity}, have no causal relevance for the model's decision \citep{Termine2023XAI}.
%Such a verification task can be solved by checking that the model's predictions are robust (i.e., do not change) under variations that affect sensitive attributes.
%That is, it ultimately involves the calculation of interventional and counterfactual questions, such as ``what will the model's decision be if I change the concept \emph{gender} from male to non-binary?''.
%
%*** Causal opacity is more on
%\emph{trustworthy} and \emph{explainable} AI systems \cite{Adadi2018, Minh2022, Beckers2022} ***
%In recent years, a plethora of techniques have been proposed 
%
to address causal opacity issues developed within the research programme of \emph{eXplainable AI} (XAI) \citep{Guidotti2018, Adadi2018, arrieta2020explainable}.
%and support a user's causal understanding of a DL model's inferences.
Among the most popular we find \emph{counterfactual explanation} (CE) methods \citep{wachter2017counterfactual}: procedures that take in input an opaque model $f$, an instance $\mathbf{x}$, and a desired prediction $y$, and return a \emph{counterfactual instance} $\mathbf{x}^\prime$ such that $f(\mathbf{x}^\prime) = y$ and the distance between $\mathbf{x}$ and $\mathbf{x}^\prime$ (according to some predefined metric) is minimal \citep{Guidotti2022}.
%CE methods promise to aid users in addressing interventional and counterfactual questions but suffer 
Although promising, CE methods capture only a week form of counterfactual dependence, sometimes referred to as \emph{direct counterfactual dependence} \citep{Beckers2022}, which assumes all the features to be causally independent with one another and directly related to the target prediction (see, \textcolor{red}{Fig. ***}).
This is an oversimplification of the causal structure of an inference, which is typically far more complex and encompasses a dense network of causal dependencies among various (from low to high-level) features.
%In particular, the predictions of a DL model typically depend causally on only a subset of the features involved, which in turn are predicted by (and thus causally depend on) other features in an iterative sequence that leads back to a subset of primitive features the model infers directly from the raw data.

Alternative to CE methods, there exist several \emph{causal features attribution} techniques that focus on measuring the \emph{causal relevance}\footnote{For example, defined in terms of Pearl's probability of sufficiency and necessity \cite{Tian2000}.} of each model's input feature for a given target prediction \textcolor{red}{*** here I will add some references ***}.
Although these techniques are promising, the focus on ``raw'' input features limit their applicability, especially to unstructured data (e.g., images)
%\footnote{The same limitation applies also to standard CEs, such as \cite{wachter2017counterfactual}.}.
%Indeed, 
whose input features denote low-level attributes (e.g., pixels) that do not typically possess an understandable and contextually-relevant meaning.
For this reason, many authors stress that good causal explanations should be \emph{concept-based}, i.e., they should rely on the ``high-level'' features (here called \emph{concepts}) a model infers form raw-data and uses as proxies for prediction \cite{Scholkopf2021, DeOliveira2024}.
However, although \emph{concept-based} explainability techniques are becoming increasing popular in XAI, so far there are very few works that aim at matching them with the requirements of causal explainability.
An example is the recent work by \citet{DeOliveira2024}, which introduces ``DiConStruct'', a causal concept-based explainability procedure based on \emph{surrogate
%\footnote{In XAI, a surrogate model is an explainable model that emulates, either globally or locally, the predictive behaviour of a black box \cite{Guidotti2018}.} 
causal models}.
First, given a black box $f$ trained on a dataset $\mathcal{D}$, DiConStruct applies causal-discovery techniques to $\mathcal{D}$ for learning a causal-graph over a set of high-level concepts. Then, it augments the graph to a \emph{Structural Causal Model} (see, \cite{Pearl2009}) and makes its predictions to converge to those of the black box $f$.
The procedure can be seen as a special instance of \emph{Post-hoc} explainability methods with surrogate models, a family of XAI techniques that generate explanations by learning a surrogate explainable model which (locally or globally) emulates the predictive behaviour of an original black box \cite{Guidotti2018, Adadi2018, Panigutti2020}. 
Although very popular, these XAI techniques incur some methodological limitations, related in particular to using surrogate model's inferences as \emph{explanantes} of the black box's behaviour. In fact, the convergence between the predictive behaviour of the surrogate model and the predictive behaviour of the black box does not \emph{per-se} guarantee that the logical-inferential structure of the two models is similar: the same predictive behaviour is indeed compatible with different logic-inference structures.
The same criticism can be applied to the methodology proposed in \cite{DeOliveira2024}.
%: the convergence between the predictive behaviour of the surrogate model and the predictive behaviour of the black box does not guarantee that there is a similarity between the causal structure of the inferences that two models provide.
Furthermore, the paper seems to make a confusion between the two problems of causal opacity and causal discovery mentioned above.
By applying causal discovery techniques, indeed, the procedure obtains a causal model \emph{of the world}, which is then used as a proxy for explaining the causal structure \emph{of the black box's inferences}.



%Among the most popular we find \emph{counterfactual explanation} (CE) methods \citep{wachter2017counterfactual}.
%A CE is an algorithm that takes an opaque model $f$, an instance $\mathbf{x}$, and a desired prediction $y$ and returns a \emph{counterfactual instance} $\mathbf{x}^\prime$ such that $f(\mathbf{x}^\prime) = y$ and the distance between $\mathbf{x}$ and $\mathbf{x}^\prime$ (according to some predefined metric) is minimal \citep{Guidotti2022}.
%CE methods promise to aid users in addressing interventional and counterfactual questions but suffer from severe limitations that ultimately undermine their reliability.
%In particular, CEs capture only a week form of counterfactual dependence, sometimes referred to as \emph{direct counterfactual dependence} \citep{Beckers2022}, which assumes all the features to be causally independent with one another and directly related to the target prediction (see, \textcolor{red}{Fig. ***}).
%This is an oversimplification of the causal structure of a DL model's inference, which is typically far more complex and encompasses a dense network of causal dependencies among various (from low to high-level) features.
%In particular, the predictions of a DL model typically depend causally on only a subset of the features involved, which in turn are predicted by (and thus depend on) other features in an iterative sequence that leads back to a subset of primitive features the model infers directly from the raw data (see, \textcolor{red}{Fig. ***}). 
%
%Making this causal structure (typically ``hidden'' within the deep network's latent space) explicit represents the first step towards causal understanding of DL models' inferences and behaviours. 
%
%\textcolor{red}{*** to decide whether to place this section here or in the background, I like it here as it fit the narrative but it can be easily moved, discuss this issue on Monday ***}
%In the literature, there are some techniques that attempt to solve this problem by following the methodology of \emph{post-hoc} explainability based on \emph{surrogate models}, which roughly relies on learning a surrogate explainable model that emulates the ``original'' black box model's inferential behaviour either locally or globally \cite{Guidotti2018}.
%For example, the procedure proposed in \citet{DeOliveira2024} 
%
%
%
%to address this task following the methodology of \emph{post-hoc} explainability based on \emph{surrogate models} \citep{Bodria2023}.
%\textcolor{red}{***check*** In particular, the proposed technique works as follows. First, they apply causal discovery algorithms to learn a ``surrogate'' causal-graphical model (CG) from the same data sample on which the original (target) DL model has been trained. Hence, they iteratively adjust the CG's predictions so to maximise their matching with the original DL models' predictions.}
%This technique has severe limitations in terms of explanatory power, in particular because explanations are generated using a surrogate CG whose similarity to the original model is obtained simply by the convergence of its predictions with those of the original model. There is therefore no guarantee that the structure of the surrogate CG really reflects the causal structure of the target model, since different causal structures are compatible (i.e. imply the same predictive behaviour).
%Furthermore, this technique \textcolor{red}{*** I will continue tomorrow, please do not touch this last part ***}


%\nb{Idea of pitch (feel free to modify):}
    % \item AI has already had a pervasive impact on many fields.
    % \item However, we still see a limited impact of AI in high-stakes domains (healthcare, autonomous driving, public administration)
    % \item Would you endorse laws written by Large Language Models (LLMs) embedded with potentially unknown biases against minorities and cultures? + another example? As of now, a cautious stance prevails, and rightly so


%one of the key limitations that prevent this from happening is that modern AI models are not interpretable, hence they are not easily controllable, nor verifiable, and therefore not certifiable (certifiable AI paper)

%how can we scientifically prove and verify this then?

%these models are opaque, in particular: causal opacity, limits control over the model and certifiability

%one way is via standard XAI counterfactuals, but: but concepts are assumed to be independent and all directly causally connected with the label (cite Molnar Interpretable ML)

%for instance, generating counterfactuals for CBMs falls in this category (i.e., interpretable but causally opaque) [cite CF CBMs]
    
%to solve this, we argue that a causal model is needed. In particular, we need (i) a causal graph specifying causal relationships between human-understandable units of information (i.e., ``concepts''), if we want interventional level interactions, and (ii) a Structural Causal Model (SCM), if counterfactual level interactions are desired (Pearl).

%discuss and introduce examples of finding an SCM in a post-hoc manner, but mention limits of finding the SCM of a decision-making process in a post-hoc manner (DiConStruct, MALESCAMO). Some of the problems include: (1) need interpretable concepts anyway, (2) surrogate dataset is not optimal to capture the decision-making process of the original model

In this paper, we present an innovative procedure to
address concept-based causal explanability that overcomes the limitations of the aforementioned existing methods. Our technique is based on \emph{Concept Bottelneck Models} (CBMs), a class of DL architectures increasingly involved in the XAI domain to deliver models that are concept-based explainable \emph{by design}.
In particular, the paper introduces \emph{Causal} CBMs, an extension of CBM delivering inferences whose causal structure:
\begin{enumerate}
    \item is transparent by design; and
    \item resembles the causal structure of the world.
\end{enumerate}
Property (1) ensures causal CBMs to be analysable via interventional and counterfactual tests, thus allowing to verify, for instance, their counterfactual fairness.
Property (2), on the other hand, ensures causal CBMs to deliver more robust and generalisable predictions, which remain accurate also under distribution shifts. 
Furthermore, in the paper we show that the adoption of a causally-explainable by design architecture does not affect the predictive performance of the models, which remain comparable to that of standard (not causally-explainable) CBMs and other black boxes.
%This also responds to the argument raised in \cite{DeOliveira2024}, according to which the use of post-hoc explainability methods is preferable, since the use of explainable-by-design architectures necessarily implies a reduction in the predictive performance of the models.


